Sitatapatra: Blocking the Transfer of Adversarial Samples

Convolutional Neural Networks (CNNs) are widely used to solve classification tasks in computer vision. However, they can be tricked into misclassifying specially crafted `adversarial' samples -- and samples built to trick one model often work alarmingly well against other models trained on the same task. In this paper we introduce Sitatapatra, a system designed to block the transfer of adversarial samples. It diversifies neural networks using a key, as in cryptography, and provides a mechanism for detecting attacks. What's more, when adversarial samples are detected they can typically be traced back to the individual device that was used to develop them. The run-time overheads are minimal permitting the use of Sitatapatra on constrained systems.

==> tables/attribution.tex <==
\begin{table}[]
\begin{adjustbox}{scale=0.8,center}
\begin{tabular}{@{}l|lll|lll@{}}
\toprule
&\multicolumn{3}{c|}{FGSM}&\multicolumn{3}{c}{FGSM+DeepFool+C\&W}\\
Polynomial         & Precision & Recall & F1   & Precision & Recall & F1   \\\midrule
$0.1x^2-1x+2 < 3$  & \textbf{0.90}      & \textbf{0.90}   & 0.90 & 0.81      & 0.29   & 0.43 \\
$x^2-22x+120 < 10$ & \textbf{0.90}      & \textbf{0.89}   & 0.90 & \textbf{0.85}      & 0.28   & 0.42 \\
$2x^2+3x+5 < 6$    & 0.53      & 0.72   & 0.61 & 0.34      & 0.33   & 0.33 \\
$2x^2+4x+5 < 6$    & 0.56      & 0.35   & 0.43 & 0.30      & 0.69   & 0.41 \\ \midrule
Micro F1           & 0.72      & 0.72   & 0.72 & 0.40      & 0.40   & 0.40 \\
Macro F1           & \textbf{0.72}      & 0.72   & 0.71 & \textbf{0.57}      & 0.40   & 0.40 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Key attribution based on the adversarial sample produced.}
\label{tab:key_attribution}
\end{table}


==> tables/dmcc.tex <==
\begin{table*}[]
\centering

\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|lllllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&         & \multicolumn{3}{c}{LeNet5}   & \multicolumn{3}{c}{MCifarNet} & \multicolumn{3}{c}{ResNet18-Cifar10}       \\
& Params  &Source   &Target   &$\Delta$  &Source   &Target   &$\Delta$   &Source  &Target  &$\Delta$ \\ \midrule
Clean
 &        &99.13    &99.09    &-         &89.04    &89.12    &-               &         &92.51    &- \\ \midrule
\multirow{3}{*}{FGSM}
 & $\epsilon=0.02$  &97.98    &92.05\\
 & $\epsilon=0.06$  &91.77    &98.13\\
 & $\epsilon=0.6$   &0.87     &2.89\\ \midrule
\multirow{2}{*}{DeepFool}
 & $i=50$           &12.40    &64.74\\
 & $i=100$          &13.96    &64.90\\ \midrule
\multirow{2}{*}{C\&W}
 &$i=100, lr=10^{-2}$   \\
 &$i=500, lr=5*10^{-3}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of adversarial samples with DMCC instrumentation.
    Source and Target are two models of the same topology but different DMCC
    instrumentations. $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of iterations for iterative methods like DeepFool
    and C\&W, $lr$ is learning rate.
    The LeNet5, MCifarNet and ResNet18-Cifar10 without defense have
    $99.03\%$, $87.56\%$ and $xx$ accuracies respectively. }
\label{tab:reg-effect}
\end{table*}


==> tables/lenet.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|lllll|lllllll|lllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
& \multicolumn{5}{c}{Pretrained}
& \multicolumn{7}{c}{Static Only}
& \multicolumn{7}{c}{Combined}       \\
& Params
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$l_2$ &$l_{\infty}$
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$S_{\mathsf{Det}}$  &$T_{\mathsf{Det}}$  &$l_2$ &$l_{\infty}$
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$S_{\mathsf{Det}}$  &$T_{\mathsf{Det}}$  &$l_2$ &$l_{\infty}$    \\ \midrule
Clean &
&99.02    &99.00    &-         &-    &-
&98.70    &98.75    &-         &-    &-    &-    &-
&99.13    &99.10    &-         &-    &-    &-    &-    \\ \midrule
\multirow{3}{*}{FGSM}
 & $\epsilon=0.02$
 &97.89 &98.98 &1.09 &0.42 &0.02 &96.95 &97.89 &0.94 &0.00 &13.33 &0.35 &0.02 &96.33 &98.20 &1.88 &0.00 &0.00 &0.41 &0.02\\
 & $\epsilon=0.08$
 &91.25 &95.94 &4.69 &1.65 &0.08 &74.69 &85.55 &10.86 &0.33 &11.30 &1.37 &0.08 &82.66 &97.03 &14.38 &0.00 &0.00 &1.64 &0.08\\
 & $\epsilon=0.6$
 &0.86 &4.14 &3.28 &11.90 &0.59 &2.34 &6.48 &4.14 &50.55 &68.50 &9.52 &0.58 &0.08 &7.89 &7.81 &21.81 &8.98 &11.84 &0.59\\
 \midrule
\multirow{2}{*}{DeepFool}
 & $i=10$
 &85.62 &96.72 &11.09 &1.75 &0.41 &98.36 &98.20 &-0.16 &0.00 &26.86 &0.81 &0.21 &98.28 &98.12 &-0.16 &0.00 &0.00 &1.11 &0.26\\
 & $i=50$
 &14.45 &92.19 &77.73 &1.85 &0.44 &32.11 &96.33 &64.22 &0.34 &14.19 &0.85 &0.21 &11.56 &98.05 &86.48 &0.18 &0.00 &1.16 &0.27\\
%  & $i=10, c=0.999$
%  &85.08 &93.98 &8.91 &1.79 &0.42 &98.12 &98.05 &-0.08 &0.00 &27.78 &0.81 &0.21 &98.28 &97.97 &-0.31 &0.00 &0.00 &1.11 &0.26\\
%  & $i=50, c=0.999$
%  &0.55 &31.56 &31.02 &2.88 &0.64 &22.97 &67.66 &44.69 &0.41 &11.34 &1.03 &0.24 &1.88 &96.25 &94.38 &0.24 &0.00 &1.57 &0.35\\
 \midrule
\multirow{2}{*}{C\&W}
 &$lr=0.5$
 &3.28 &86.88 &83.59 &3.10 &0.71 &4.61 &65.94 &61.33 &19.49 &50.78 &2.95 &0.69 &4.45 &93.05 &88.59 &2.95 &4.66 &2.91 &0.69\\
 &$lr=1.0$
 &0.39 &60.39 &60.00 &4.25 &0.76 &0.86 &36.41 &35.55 &39.57 &73.93 &3.90 &0.79 &0.31 &80.62 &80.31 &6.82 &10.38 &3.95 &0.77\\
 &$lr=0.5, c=0.999$
 &3.52 &16.09 &12.58 &5.12 &0.90 &5.16 &8.75 &3.59 &68.86 &93.14 &4.91 &0.94 &4.77 &41.48 &36.72 &15.51 &28.48 &4.89 &0.92\\
 &$lr=1.0, c=0.999$
 &0.47 &5.86 &5.39 &5.78 &0.95 &1.56 &1.88 &0.31 &86.03 &96.74 &5.71 &0.98 &0.55 &24.61 &24.06 &25.37 &37.03 &5.49 &0.97\\


\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of LeNet5 on MNIST with different instrumentations.
    Source generates adversarial samples and Target got attacked.
    S-Acc and T-Acc are the accuracies of the Source and Target
    with adversarial samples respectively, and $\Delta$ is the difference
    in accuracies.
    $l_2$ and $l_{\infty}$ are
    the averaged $l_2$ and $l_{\infty}$ norms of
    the distortions on input images.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of steps for DeepFool,
    $lr$ is learning rate for C\&W.
    $c$ is the confidence, the adversarial sample has to cause
    the misclassified class to have a probability above this threshold.
    We use $20$ steps on C\&W, and the polynomial parameters for
    source and target models are [2, 3, 5, 6] and [2, 4, 5, 6]
    respectively.
    }
\label{tab:lenet}
\end{table*}

% &0.03515625 &0.1609375 &0.12578125 &- &- &5.11747989654541 &0.9028810620307922 &0.0515625 &0.0875 &0.0359375 &0.688584886106417 &0.931417603453999 &4.913985252380371 &0.9375062108039856 &0.04765625 &0.41484375 &0.3671875 &0.15508982651794906 &0.2848341580612277 &4.892731952667236 &0.9236176252365113\\
% &0.0046875 &0.05859375 &0.05390625 &- &- &5.780204486846924 &0.9455502033233643 &0.015625 &0.01875 &0.0031249999999999993 &0.8602972176238735 &0.967354598976778 &5.706935977935791 &0.9802315831184387 &0.00546875 &0.24609375 &0.240625 &0.2537238738999537 &0.37032561285154997 &5.494970989227295 &0.9740454196929932\\
% &0.00546875 &0.315625 &0.31015624999999997 &- &- &2.878287172317505 &0.6448896765708924 &0.2296875 &0.6765625 &0.44687499999999997 &0.004097492259764338 &0.11343711671285042 &1.0265390157699585 &0.24413472414016724 &0.01875 &0.9625 &0.94375 &0.0023873015873015872 &0.0 &1.569072151184082 &0.3500462770462036\\
% &0.85078125 &0.93984375 &0.08906249999999993 &- &- &1.7868361949920655 &0.4234331727027893 &0.98125 &0.98046875 &-0.0007812499999999556 &0.0 &0.2777777777777778 &0.8148597121238709 &0.20861342549324036 &0.9828125 &0.9796875 &-0.0031249999999999334 &0.0 &0.0 &1.1136931896209716 &0.2616474211215973\\


==> tables/overhead.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{scale=0.8}
\begin{tabular}{l|lllll}
    \toprule
    \multirow{2}{*}{Model}
        & \multicolumn{5}{c}{{\#FLOPs}} \\
    {}
        & original & detector & guard
        & total & overhead \\
    \midrule
    LeNet5
        & 480,500 & 28,160 & 7,660
        & 516,320 & 7.45\% \\
    ResNet18
        & 37,016,576 & 152,094 & 1,847,106
        & 39,015,776 & 5.40\% \\
    MCifarNet
        & 174,301,824 & 715,422 & 646,082
        & 175,663,328 & 0.64\% \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{%
    The computational costs,
    measured in the number of FLOPs,
    added by the detector and guard modules
    to the original network.
}\label{tab:overhead}
\end{table}


==> tables/penalty.tex <==
\begin{table}

\begin{adjustbox}{width=0.4\linewidth,center}
\begin{tabular}{@{}l|lll@{}}
\toprule
           & $l_2$        & $l_{\infty}$    & Det (\%) \\ \midrule
$\alpha=1$ & \textbf{1.38} & 0.22 & 6 \\
$\alpha=0$ & 1.29 & \textbf{0.24} & 7 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{C-LBFGS generated perturbations with and without penalty for detection}
\label{tab:ataku}
\end{table}


==> tables/taboo.tex <==
\begin{table*}[!h]
\centering

\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|llllll|llllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&
& \multicolumn{6}{c}{LeNet5}
& \multicolumn{6}{c}{MCifarNet}
\\
& Params
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
\\ \midrule
Clean&
&99.13    &99.25    &-             &-       &-            &-
&89.51    &90.14    &-             &-       &-            &-
\\ \midrule
\multirow{4}{*}{FGSM}
& $\epsilon=0.02$
&97.58 &99.45 &1.87 &0.00 &0.35 &0.02
&10.70 &21.41 &10.70 &1.41 &0.95 &0.02
\\
& $\epsilon=0.06$
&82.58 &98.36 &15.78 &0.00 &1.37 &0.08
&2.27 &11.17 &8.91 &10.47 &3.49 &0.06
\\
& $\epsilon=0.6$
&2.89 &13.67 &10.78 &0.19 &9.53 &0.58
&0.78 &9.22 &8.44 &78.63 &20.06 &0.46
\\
& mean
&- &- &9.48 &0.06 &- &-
&- &- &9.35 &30.17 &- &-
\\
\midrule
\multirow{3}{*}{DeepFool}
& $i=50$
&21.09 &99.30 &78.20 &0.00 &1.05 &0.25
&0.23 &69.53 &69.30 &2.49 &0.25 &0.03
\\
& $i=10$
&98.44 &99.45 &1.02 &0.00 &1.01 &0.25
&0.39 &69.53 &69.14 &2.49 &0.25 &0.03
\\
& mean
&- &- &39.61 &0.00 &- &-
&- &- &69.22 &2.49 &- &-
\\ \midrule
\multirow{3}{*}{C\&W}
&$lr=0.5$
&6.33 &97.34 &91.02 &0.00 &3.01 &0.70
&4.06 &11.33 &7.27 &89.25 &9.43 &0.24
\\
&$lr=1.0$
&1.41 &91.80 &90.39 &0.95 &3.99 &0.79
&9.45 &14.45 &5.00 &88.86 &16.33 &0.41
\\
& mean
&- &- &90.70 &0.48 &- &-
&- &- &6.14  &89.10 &- &-
\\
\midrule
% \multirow{2}{*}{C\&W $c=0.999$}
C\&W
&$lr=0.5$
&6.64 &64.14 &57.50 &2.38 &4.89 &0.92
&5.08 &3.59 &-1.48 &100.00 &17.95 &0.67
\\
$c=0.999$
&$lr=1.0$
&1.95 &46.95 &45.00 &6.47 &5.53 &0.97
&10.86 &7.50 &-3.36 &100.00 &22.87 &0.76
\\
& mean
&- &- &51.25 &4.43 &- &-
&- &- &-2.42  &100.00 &- &-
\\
\midrule
Mean
&
&- &- &43.50 &1.11 &- &-
&- &- &19.32 &52.62 &- &-
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of LeNet5 and MCifarNet
    with SCM (using Guard only).
    Source and Target are two models of the same topology but different
    SCM instrumentations.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of iterations and $lr$ is the learning rate.}
    % The LeNet5, MCifarNet, ResNet18-Cifar10 and ResNet18-Cifar100
    % without instrumentations have
    % $99.03\%$, $87.56\%$, $xx$ and $xx$ accuracies respectively. }
\label{tab:taboo}
\end{table*}

